Mining Parametric Temporal Logic Properties in Model Based Design for Cyber-Physical Systems

One of the advantages of adopting a Model Based Development (MBD) process is that it enables testing and verification at early stages of development. However, it is often desirable to not only verify/falsify certain formal system specifications, but also to automatically explore the properties that the system satisfies. In this work, we present a framework that enables property exploration for Cyber-Physical Systems. Namely, given a parametric specification with multiple parameters, our solution can automatically infer the ranges of parameters for which the property does not hold on the system. In this paper, we consider parametric specifications in Metric or Signal Temporal Logic (MTL or STL). Using robust semantics for MTL, the parameter mining problem can be converted into a Pareto optimization problem for which we can provide an approximate solution by utilizing stochastic optimization methods. We include algorithms for the exploration and visualization of multi-parametric specifications. The framework is demonstrated on an industrial size, high-fidelity engine model as well as examples from related literature.

==> peFramework.tex <==
\section{Parameter Estimation Framework}

- non-monotonic specifications
- large number of parameters strategy - split up the formula in conjunctive parts
- 

==> questionsGeorgios.tex <==
- Change of name justification
- Rev 1 comment 5
- Abstract (STL or MTL). Also added statement about STL in intro.
- Cite also the 2006 conf. version ??? Comments
- Check pareto front reference
- Check itemization specifications
- To enable of elicitation of formal requirements for CPS, tools such as \textsc{ViSpec} \cite{hoxhavispec} may be utilized. 
- In this example, the output of the system is the state of the system
- HS example
- That is, the solution to the multi-parameter mining problem is in the form of a Pareto front. citation???
- Page 4 comment to add 1st conf. papaer.
- IMPORTANT: COMMENT ABOUT HS EXAMPLE IN FIG. 1
- Case (ii) is symmetric with respect to the temporal operator and lemma \ref{lem:timeOperMonInc} is symmetric in terms of monotonicity.
- FIX BOLD Y ISSUES EX 4
- Update funding source
- if we have time make figure for proposition 2
- parameter falsification domain - expanding or reducing?
- Algorithm 1 set to zeros
- Dimension alg 1
- Alg 1 questionmarks
- Namely, the choice of $\vec{b}$ directs the expansion of the parameter falsification domain along a specific vector.
- Algorithm 2

TODO: FIX COMMENT IN FIRST PAGE LAST
